Monitoring and Diagnosability of Perception Systems

Perception is a critical component of high-integrity applications of robotics and autonomous systems, such as self-driving vehicles. In these applications, failure of perception systems may put human life at risk, and a broad adoption of these technologies requires the development of methodologies to guarantee and monitor safe operation. Despite the paramount importance of perception systems, currently there is no formal approach for system-level monitoring. In this work, we propose a mathematical model for runtime monitoring and fault detection and identification in perception systems. Towards this goal, we draw connections with the literature on diagnosability in multiprocessor systems, and generalize it to account for modules with heterogeneous outputs that interact over time. The resulting temporal diagnostic graphs (i) provide a framework to reason over the consistency of perception outputs -- across modules and over time -- thus enabling fault detection, (ii) allow us to establish formal guarantees on the maximum number of faults that can be uniquely identified in a given perception system, and (iii) enable the design of efficient algorithms for fault identification. We demonstrate our monitoring system, dubbed PerSyS, in realistic simulations using the LGSVL self-driving simulator and the Apollo Auto autonomy software stack, and show that PerSyS is able to detect failures in challenging scenarios (including scenarios that have caused self-driving car accidents in recent years), and is able to correctly identify faults while entailing a minimal computation overhead (< 5 ms on a single-core CPU).

==> sections/app-cc-perception.tex <==
%!TEX root = ../main.tex

\section{Consistency Test for Object Detection}

\cref{alg:cc_perception} shows the pseudocode of a a typical object detection consistency test.
The function $\mathrm{FOV}(A)$ returns the set of obstacles that are i the field-of-view of the sensor $A$.
The operator $\approxin$ represent an approximate set membership operator, it is needed as obstacles detected by different sensors might might partially overlap but still being the same obstacle.
We implement this checks as area overlap between convex hulls, but other choices are possible.
The function $T_B^W(o)$ takes an obstacle in body frame and transforms it to the world frame.
Finally, the function $\mathrm{InCurrentLane(o)}$ takes an obstacle in the world frame and returns \emph{True} if it within the lane occupied byt the AV.

In the \emph{For} loops starting at lines \ref{line:ccp_obstaclesA} and \ref{line:ccp_obstaclesB} we create the list of unmatched obstacles $U$.
We consider an unmatched obstacle $o\in\obs{A}$ an obstacle that is detected by sensor $A$, that is within sensor $B$ field-of-view but that $B$ failed to detect, and vice versa.
If there is any unmatched obstacle (line~\ref{line:cpp_nonempty_unmatched}) we compute the severity level (high for obstacle on the lane, low otherwise) and return, otherwise we return \emph{PASS} (no fault).

\begin{algorithm}[t]
	\caption{Object Detection Consistency Test}
	\SetAlgoLined
    \KwIn{$\obs{A}$ obstacles detected by $A$ in the body frame; $\obs{B}$ obstacle detected by $B$ in the body frame.}
	\KwOut{NO_FAULT, LOW or HIGH.}
  \BlankLine
  $U=\emptyset$\;
  \For{$o\in\obs{A}$\label{line:ccp_obstaclesA}}{ 
    \If{$o\in\mathrm{FOV}(B)$ and $z\not\approxin\obs{B}$}{
      $U=U\cup \{o\}$\;
    }
  }
  \For{$o\in\obs{B}$\label{line:ccp_obstaclesB}}{ 
    \If{$o\in\mathrm{FOV}(A)$ and $z\not\approxin\obs{A}$}{
      $U=U\cup \{o\}$\;
    }
  }
  \If{|U| > 0}{ \label{line:cpp_nonempty_unmatched}
    \For{$o\in U$}{
      \If{$\mathrm{InCurrentLane(T_B^W(o))}$}{
        \Return{HIGH}
      }
      \Return{LOW}
    }
  }
  \Return{PASS}
  \label{alg:cc_perception}
\end{algorithm}




==> sections/figures/tesla_crash.tex <==
%!TEX root = ../../main.tex

\begin{figure*}[ht!]
  \vspace{5mm}
	\begin{center}
	\begin{minipage}{\textwidth}
	\begin{tabular}{ccc}%
    \mpPreSpace
			\begin{minipage}{\mpColTwo}%
        \centering%
        \includegraphics[width=\columnwidth]{scenario_lgsvl.jpg} \\
			\end{minipage}
		& \mpMidSpaceTwo
			\begin{minipage}{\mpColTwo}%
        \centering%
        \includegraphics[width=\columnwidth]{tesla_crash.jpg} \\
			\end{minipage}
		\end{tabular}
	\end{minipage}
	\mpPostSpace
  \caption{ {\bf Simulated scenario.} (a) Simulated scenario in \lgsvl, (b) Real Tesla autopilot crash in Taiwan}
	\label{fig:tesla_crash}
	\end{center}
\end{figure*}

% \begin{figure}[ht!]
%   \includegraphics[width=\linewidth]{traffic_3_lgsvl.jpg}
%   \centering
%   \caption{{\bf Scenario.} The \lgsvl scenario, an overturned truck on lane.}
%   \label{fig:lgsvl_scenario}
% \end{figure}

==> sections/figures/trajectories.tex <==
%!TEX root = ../../main.tex

\begin{figure*}[ht!]
	\begin{center}
	\begin{minipage}{\textwidth}
	\begin{tabular}{ccc}%
		\mpPreSpace
			\begin{minipage}{\mpColTwo}%
        \centering%
        \includegraphics[width=\columnwidth]{perception_trajectory} \\
			\end{minipage}
		& \mpMidSpaceTwo
			\begin{minipage}{\mpColTwo}%
        \centering%
        \includegraphics[width=\columnwidth]{gps_trajectory} \\
			\end{minipage}
		\end{tabular}
	\end{minipage}
	\mpPostSpace
  \caption{ {\bf Trajectories.} (a) Object detection, (b) Vehicle localization. Red represent high severity fault, yellow low severity, green no fault.}
	\label{fig:trajectories}
	\vspace{-5mm} 
	\end{center}
\end{figure*}

